Expanding the High-z Supernova Frontier: "Wide-Area" JWST Discoveries from the First Two Years of COSMOS-Web

Transient astronomy in the early Universe (z > 2) remains largely unexplored, lying beyond the rest-frame optical spectroscopic reach of most current observatories. Yet this regime promises transformative insights, with high-redshift transients providing direct access to the early Universe and enabling studies of how stellar populations and cosmology evolve over cosmic time. JWST is uniquely equipped to probe these redshifts efficiently in the rest-frame optical and near-IR. We present results from an initial pathfinder search, covering an area of ~133 arcmin^2 (~0.037 deg^2) independently imaged by the PRIMER and COSMOS-Web (hereafter COSMOS) extragalactic surveys. Although neither program was designed for time-domain astronomy, combining their data results in difference images separated by roughly one year, leading to the discovery of 68 supernovae (SNe) with host photometric redshifts reaching z < 5. For most SNe, only a single epoch is available, but the combination of host redshift, classification, color, and magnitude enables us to prioritize candidates for detailed photometric and spectroscopic follow-up. Among the most notable sources are a relatively bright, blue CCSN at z > 3 (SN 2023aeab) and a young, normal SN Ia at z > 2 (SN 2023aeax). The sample distribution highlights the increasing likelihood that a wide-area JWST program can uncover younger, bluer, and potentially more extreme explosions. While this pathfinder effort is limited in cadence and number of filters, it demonstrates the strong potential of a dedicated, well-planned time-domain survey with JWST to obtain the sample sizes and rate measurements needed to chart SN populations deep into the early Universe.

==> acknowledgements.tex <==
Some/all of the data presented in this paper were obtained from the Mikulski Archive for Space Telescopes (MAST) at the Space Telescope Science Institute. The specific observations analyzed can be accessed via \dataset[https://doi.org/10.17909/n7kq-ef83]{https://doi.org/10.17909/n7kq-ef83}. STScI is operated by the Association of Universities for Research in Astronomy, Inc., under NASA contract NAS5–26555. Support to MAST for these data is provided by the NASA Office of Space Science via grant NAG5–7584 and by other grants and contracts. The STScI TSST group acknowledges partial support from  JWST-GO-06541, JWST-GO-06585, and JWST-GO-05324. This work was made possible by utilising the CANDIDE cluster at the Institut d’Astrophysique de Paris. The cluster was funded through grants from the PNCG, CNES, DIM-ACAV, the Euclid Consortium, and the Danish National Research Foundation Cosmic Dawn Center (DNRF140). It is maintained by Stephane Rouberol. GEM acknowledges the Villum Fonden research grants 37440 and 13160. The Cosmic Dawn Center (DAWN) is funded by the Danish National Research Foundation under grant DNRF140. This project has received funding from the European Union’s Horizon 2020 research and innovation programme under the Marie Skłodowska-Curie grant agreement No 101148925. The French contingent of the COSMOS team is partly supported by the Centre National d'Etudes Spatiales (CNES). SF acknowledges support from the Dunlap Institute, funded through an endowment established by the David Dunlap family and the University of Toronto. ODF acknowledges the use of ChatGPT in helping with minor phrasing, grammar, and editing, as well as with generating some tables and figures. DBS gratefully acknowledges support from NSF Grant 2407752. MRS is supported by an STScI Postdoctoral Fellowship. JP is supported by NASA through a Einstein Fellowship grant No. HF2-51541.001 awarded by the Space Telescope Science Institute (STScI), which is operated by the Association of Universities for Research in Astronomy, Inc., for NASA, under contract NAS5-26555. Y.Z. Acknowledges support from the MAOF grant 12641898 and visitor support from the Observatories of the Carnegie Institution for Science, Pasadena, CA, where part of this work was completed. N.E.D acknowledge support from NSF grants LEAPS-2532703  and AST-2510993. 



==> authors.tex <==
\author[0000-0003-2238-1572]{Ori D.Fox}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\email{ofox@stsci.edu}

\author[0000-0002-4410-5387]{Armin Rest}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\affiliation{William H. Miller III Department of Physics \& Astronomy, Johns Hopkins University, 3701 San Martin Dr, Baltimore, MD 21218, USA}
\email{arest@stsci.edu}

\author[0000-0002-2361-7201]{Justin~D.~R.~Pierel}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\altaffiliation{NASA Einstein Fellow}
\email{jpierel@stsci.edu}

\author[0000-0003-4263-2228]{David~A.~Coulter}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\email{dcoulter@stsci.edu}

\author[0000-0002-0930-6466]{Caitlin M. Casey}
\email{cmcasey@ucsb.edu}
\affiliation{Department of Physics, University of California, Santa Barbara, Santa Barbara, CA 93106, USA}
\affiliation{Cosmic Dawn Center (DAWN), Jagtvej 128, DK2200 Copenhagen N, Denmark}

\author[0000-0001-9187-3605]{Jeyhan S. Kartaltepe}
\email{jeyhan@astro.rit.edu}
\affiliation{Laboratory for Multiwavelength Astrophysics, School of Physics and Astronomy, Rochester Institute of Technology, 84 Lomb Memorial Drive, Rochester, NY 14623, USA}
\email{jeyhan@astro.rit.edu}

\author[0000-0003-3596-8794]{Hollis B. Akins}
\email{hollis.akins@gmail.com}
\altaffiliation{NSF Graduate Research Fellow}
\affiliation{Department of Astronomy, The University of Texas at Austin, 2515 Speedway Blvd Stop C1400, Austin, TX 78712, USA}

\author[0000-0002-3560-8599]{Maximilien Franco}
\email{maximilien.franco@cea.fr}
\affiliation{Université Paris-Saclay, Université Paris Cité, CEA, CNRS, AIM, 91191 Gif-sur-Yvette, France}
\email{francomaximilien@gmail.com}

\author[0000-0003-0209-674X]{Mike~Engesser}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\email{mengesser@stsci.edu}

\author[0000-0003-2037-4619]{Conor~Larison}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\email{clarison@stsci.edu}

\author[0000-0003-1169-1954]{Takashi~J.~Moriya}
\affiliation{National Astronomical Observatory of Japan, National Institutes of Natural Sciences, 2-21-1 Osawa, Mitaka, Tokyo 181-8588, Japan} 
\affiliation{Graduate Institute for Advanced Studies, SOKENDAI, 2-21-1 Osawa, Mitaka, Tokyo 181-8588, Japan}
\affiliation{School of Physics and Astronomy, Monash University, Clayton, VIC 3800, Australia}
\email{takashi.moriya@nao.ac.jp}

\author[0000-0001-9171-5236]{Robert M. Quimby} 
\affiliation{Department of Astronomy and Mount Laguna Observatory, \\ San Diego State University, San Diego, CA 92182, USA} 
\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, The University of Tokyo, Kashiwa, Chiba 277-8583, Japan}
\email{rquimby@sdsu.edu}

\author[0000-0002-7087-0701]{Marko Shuntov}
\email{marko.shuntov@nbi.ku.dk}
\affiliation{Cosmic Dawn Center (DAWN), Jagtvej 128, DK2200 Copenhagen N, Denmark}
\affiliation{Niels Bohr Institute, University of Copenhagen, Jagtvej 128, DK-2200, Copenhagen, Denmark}
\affiliation{University of Geneva, 24 rue du Général-Dufour, 1211 Genève 4, Switzerland}
\email{marko.shuntov@nbi.ku.dk}

\author[0000-0003-2445-3891]{Matthew~R.~Siebert}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\email{msiebert@stsci.edu}

\author[0000-0002-4781-9078]{Christa DeCoursey}
\affiliation{Steward Observatory, University of Arizona, 933 N. Cherry Ave, Tucson, AZ 85721, USA}
\email{cndecoursey@arizona.edu}

\author[0000-0001-5281-731X]{Rodrigo Angulo}
\affiliation{William H. Miller III Department of Physics \& Astronomy, Johns Hopkins University, 3701 San Martin Dr, Baltimore, MD 21218, USA}
\email{rangulo1@jhu.edu}

\author[0000-0002-7566-6080]{James~M.~DerKacy}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\email{jderkacy@stsci.edu}

\author[0000-0003-4761-2197]{Nicole E. Drakos}
\email{ndrakos@hawaii.edu}
\affiliation{Department of Physics and Astronomy, University of Hawaii, Hilo, 200 W Kawili St, Hilo, HI 96720, USA}
\email{ndrakos@hawaii.edu}

\author[0000-0003-1344-9475]{Eiichi Egami}
\affiliation{Steward Observatory, University of Arizona, 933 N. Cherry Ave, Tucson, AZ 85721, USA}
\email{egami@arizona.edu}

 \author[0000-0001-8519-1130]{Steven L. Finkelstein}
 \affiliation{Department of Astronomy, The University of Texas at Austin, 2515 Speedway Blvd Stop C1400, Austin, TX 78712, USA} 
\affiliation{Cosmic Frontier Center, The University of Texas at Austin, Austin, TX, USA} 
\email{stevenf@astro.as.utexas.edu}

\author[0009-0000-0272-5468]{Carter Flayhart}
\email{cbf2388@rit.edu}
\affiliation{Laboratory for Multiwavelength Astrophysics, School of Physics and Astronomy, Rochester Institute of Technology, 84 Lomb Memorial Drive, Rochester, NY 14623, USA}

\author[0000-0001-7201-5066]{Seiji Fujimoto}
\affiliation{David A. Dunlap Department of Astronomy and Astrophysics, University of Toronto, 50 St. George Street, Toronto, Ontario, M5S 3H4, Canada} \affiliation{Dunlap Institute for Astronomy and Astrophysics, 50 St. George Street, Toronto, Ontario, M5S 3H4, Canada}
\email{seiji.fujimoto@utoronto.ca}

\author[0000-0003-0209-9246]{Estefania~Padilla~Gonzalez}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\email{epadill7@jh.edu}

\author[0000-0002-5060-1379]{Massimo~Griggio}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\email{mgriggio@stsci.edu}

\author[0000-0003-0129-2079]{Santosh Harish}
\email{harish.santosh@gmail.com}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\affiliation{Laboratory for Multiwavelength Astrophysics, School of Physics and Astronomy, Rochester Institute of Technology, 84 Lomb Memorial Drive, Rochester, NY 14623, USA}

\author[0000-0002-7303-4397]{Olivier Ilbert}
\email{olivier.ilbert@lam.fr}
\affiliation{Aix Marseille Univ, CNRS, CNES, LAM, Marseille, France}
\email{olivier.ilbert@lam.fr}

\author[orcid=0000-0000-0000-0001,sname='Inayoshi']{Kohei Inayoshi}
\altaffiliation{}
\affiliation{Kavli Institute for Astronomy and Astrophysics, Peking University, Beijing 100871, China}
\email{inayoshi@pku.edu.cn}  

\author[0000-0002-6610-2048]{Anton~M.~Koekemoer}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\email{koekemoer@stsci.edu}

\author[0000-0002-5588-9156]{Vasily Kokorev}
\affiliation{Department of Astronomy, The University of Texas at Austin, 2515 Speedway Blvd Stop C1400, Austin, TX 78712, USA}
\email{vasily.kokorev.astro@gmail.com}

\author[0009-0008-5926-818X]{Clotilde Laigle}\affiliation{Institut d’Astrophysique de Paris, UMR 7095, CNRS, and Sorbonne Université, 98bis boulevard Arago, 75014 Paris, France}
\email{clotilde.laigle@physics.ox.ac.uk}

\author[0000-0003-3216-7190]{Erini~Lambrides}
\affiliation{NASA-Goddard Space Flight Center, Greenbelt MD, 20771, USA}
\email{erini.lambrides@nasa.gov}

\author[0000-0003-2366-8858]{Rebecca L. Larson}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\email{rlarson@stsci.edu}

\author[0000-0002-0514-5650]{Xiaolong Li}
\affiliation{William H. Miller III Department of Physics \& Astronomy, Johns Hopkins University, 3701 San Martin Dr, Baltimore, MD 21218, USA}
\email{xli360@jhu.edu}

\author[0000-0001-9773-7479]{Daizhong Liu}
\email{dzliu@pmo.ac.cn}
\affiliation{Purple Mountain Observatory, Chinese Academy of Sciences, 10 Yuanhua Road, Nanjing 210023, China}
\email{dzliu@mpe.mpg.de}

\author[0000-0002-4872-2294]{Georgios~E.~Magdis}
\affiliation{Cosmic Dawn Center (DAWN), Jagtvej 128, DK2200 Copenhagen N, Denmark} \affiliation{DTU-Space, Technical University of Denmark, Elektrovej 327, 2800, Kgs. Lyngby, Denmark}
\email{geoma@space.dtu.dk}

\author[0000-0002-9883-7460]{Jacqueline E. McCleary}
\affiliation{Department of Physics, Northeastern University, 360 Huntington Ave, Boston, MA}
\email{j.mccleary@northeastern.edu}

\author[0000-0002-9489-7765]{Henry~J.~McCracken}
\affiliation{Institut d’Astrophysique de Paris, UMR 7095, CNRS, and Sorbonne Université, 98bis boulevard Arago, 75014 Paris, France}
\email{hjmcc@iap.fr}

\author[0009-0003-9297-6587]{Nicolas McMahon}
\affiliation{Laboratory for Multiwavelength Astrophysics, School of Physics and Astronomy, Rochester Institute of Technology, 84 Lomb Memorial Drive, Rochester, NY 14623, USA}
\email{njm4071@rit.edu}

\author[0000-0002-6149-8178]{Jed McKinney}
\altaffiliation{NASA Hubble Fellow}
\affiliation{Department of Astronomy, The University of Texas at Austin, 2515 Speedway Blvd Stop C1400, Austin, TX 78712, USA}
\email{jed.mckinney@austin.utexas.edu}

\author[0000-0001-8385-3727]{Thomas~Moore}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\email{tmoore@stsci.edu}

\author[0000-0003-2397-0360]{Louise Paquereau} 
\affiliation{Institut d’Astrophysique de Paris, UMR 7095, CNRS, and Sorbonne Université, 98bis boulevard Arago, 75014 Paris, France}
\email{louise.paquereau@iap.fr}

\author[0000-0002-4485-8549]{Jason Rhodes}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Drive, Pasadena, CA 91001, USA}
\email{jason.d.rhodes@jpl.nasa.gov}

\author[0000-0002-4271-0364]{Brant~E.~Robertson}
\affiliation{Department of Astronomy and Astrophysics, University of California, Santa Cruz, 1156 High Street, Santa Cruz, CA 95064, USA}
\email{brant@ucsc.edu}

\author[0000-0002-1233-9998]{David~B.~Sanders}
\affiliation{Institute for Astronomy, University of Hawai’i at Manoa, 2680 Woodlawn Drive, Honolulu, HI 96822, USA}
\email{sandersd@hawaii.edu}

\author[0009-0009-3048-9090]{Sogol~Sanjaripour}
\affiliation{Department of Physics and Astronomy, University of California Riverside, Riverside, CA 92521, USA}
\email{sogol.sanjaripour@email.ucr.edu}

\author[0000-0002-2798-2943]{Koji~Shukawa}
\affiliation{William H. Miller III Department of Physics \& Astronomy, Johns Hopkins University, 3701 San Martin Dr, Baltimore, MD 21218, USA}
\email{kshukaw1@jh.edu}

\author[0000-0002-7756-4440]{Louis-Gregory~Strolger}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\email{strolger@stsci.edu}

\author[0000-0003-3631-7176]{Sune~Toft}
\affiliation{Institute for Astronomy, University of Hawai’i at Manoa, 2680 Woodlawn Drive, Honolulu, HI 96822, USA}
\affiliation{Cosmic Dawn Center (DAWN), Jagtvej 128, DK2200 Copenhagen N, Denmark}
\affiliation{Niels Bohr Institute, University of Copenhagen, Jagtvej 128, DK-2200, Copenhagen, Denmark}
\email{sune@nbi.ku.dk}

\author[0000-0001-5233-6989]{Qinan Wang}
\affiliation{Department of Physics and Kavli Institute for Astrophysics and Space Research, Massachusetts Institute of Technology, 77 Massachusetts Avenue, Cambridge, MA 02139, USA}
\email{qnwang@mit.edu}

\author[0000-0002-3742-8460]{Robert~E.~Williams}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\email{wms@stsci.edu}

\author[0000-0002-0632-8897]{Yossef~Zenati}
\affiliation{William H. Miller III Department of Physics \& Astronomy, Johns Hopkins University, 3701 San Martin Dr, Baltimore, MD 21218, USA}
\affiliation{Astrophysics Research Center of The Open University (ARCO), Ra’anana 4353701, Israel}
\affiliation{Department of Natural Sciences, The Open University of Israel, Ra’anana 4353701, Israel}
\email{yzenati1@jhu.edu}

==> cosmos_classifications_rotated_table5.tex <==

\startlongtable
\begin{deluxetable*}{lccccccrr}
\centering
\tablecaption{COSMOS Classifications Data}
\tablehead{
\colhead{Name} & \colhead{RA} & \colhead{DEC} & \colhead{$z$} & \colhead{Brightest} & \colhead{Brightest} & \colhead{F150W} & \colhead{$\chi^2$~Ia} & \colhead{$\chi^2$~CC}\\
\colhead{(AT)} & \colhead{} & \colhead{} & \colhead{(err)} & \colhead{Mag (err)} & \colhead{Filter} & \colhead{Mag (err)} & \colhead{} & \colhead{} 
}
\label{tab:cosmos_classifications}
\startdata
2023aebb & 10:00:16.783 & +02:18:47.34 & 5.20 (0.14) & 27.80 (0.21) & F277W & -- & -- & -- \\ 
2023aebi & 10:00:21.361 & +02:10:42.55 & 4.22 (0.14) & 27.20 (0.23) & F444W & 29.40 (0.75) & -- & -- \\ 
2023aebl & 10:00:15.901 & +02:14:02.46 & 4.02 (0.14) & 26.90 (0.08) & F150W & 26.90 (0.08) & -- & -- \\ 
2023aeab & 10:00:33.363 & +02:23:44.70 & 3.55 (0.09) & 27.20 (0.09) & F115W & 27.50 (0.07) & -- & -- \\ 
2023aeaf & 10:00:22.800 & +02:22:24.61 & 3.55 (0.12) & 27.50 (0.13) & F150W & 27.50 (0.13) & 3.85 & -- \\ 
2023aeag & 10:00:29.211 & +02:22:28.53 & 3.51 (0.07) & 26.00 (0.12) & F277W & 28.10 (0.16) & -- & -- \\ 
2023adzt & 10:00:22.456 & +02:20:56.46 & 2.35 (0.16) & 27.10 (0.06) & F150W & 27.10 (0.07) & -- & 1.88 \\ 
2023aeax & 10:00:26.401 & +02:19:33.97 & 2.25 (0.10) & 26.00 (0.04) & F150W & 26.00 (0.04) & -- & -- \\ 
2023aeam & 10:00:34.227 & +02:15:09.97 & 2.18 (0.11) & 26.10 (0.04) & F150W & 26.10 (0.04) & -- & -- \\ 
2023aebk & 10:00:25.124 & +02:11:14.74 & 2.14 (0.14) & 27.00 (0.07) & F150W & 27.00 (0.07) & 1.84 & 3.82 \\ 
2023aeal & 10:00:22.698 & +02:15:01.45 & 1.90 (0.14) & 27.90 (0.22) & F150W & 27.90 (0.22) & 2.02 & -- \\ 
2023aeaa & 10:00:22.878 & +02:23:11.13 & 1.89 (0.14) & 27.40 (0.10) & F150W & 27.80 (0.15) & 2.67 & 4.03 \\ 
2023aeak & 10:00:21.473 & +02:14:53.80 & 1.88 (0.10) & 25.60 (0.04) & F115W & 26.10 (0.04) & 2.51 & -- \\ 
2023aebf & 10:00:22.782 & +02:10:31.54 & 1.75 (0.14) & 25.40 (0.11) & F277W & -- & -- & -- \\ 
2023adzw & 10:00:31.677 & +02:21:09.06 & 1.75 (0.14) & 27.30 (0.10) & F115W & 27.50 (0.08) & -- & 2.17 \\ 
2023adze & 10:00:33.547 & +02:25:42.12 & 1.70 (0.13) & 27.00 (0.10) & F115W & 27.10 (0.07) & -- & -- \\ 
2023adzi & 10:00:23.748 & +02:25:55.56 & 1.69 (0.13) & 26.70 (0.10) & F115W & 27.10 (0.07) & -- & -- \\ 
2023adyx & 10:00:43.238 & +02:26:43.05 & 1.64 (0.14) & 27.60 (0.16) & F277W & 27.70 (0.17) & -- & -- \\ 
2023aeaq & 10:00:32.498 & +02:17:07.33 & 1.61 (0.14) & 27.30 (0.08) & F150W & 27.30 (0.08) & -- & 2.50 \\ 
2023adzo & 10:00:39.312 & +02:24:54.30 & 1.52 (0.15) & 27.70 (0.13) & F277W & -- & -- & -- \\ 
2023adyy & 10:00:14.838 & +02:16:58.39 & 1.52 (0.13) & 26.60 (0.09) & F115W & 27.10 (0.10) & -- & -- \\ 
2023adzq & 10:00:25.420 & +02:20:36.49 & 1.49 (0.10) & 25.90 (0.04) & F115W & 26.00 (0.03) & -- & -- \\ 
2023aeav & 10:00:30.774 & +02:19:22.36 & 1.48 (0.10) & 27.20 (0.11) & F115W & 27.70 (0.11) & -- & 1.42 \\ 
2023adzy & 10:00:34.676 & +02:22:00.76 & 1.45 (0.13) & 27.40 (0.14) & F150W & 27.40 (0.14) & -- & -- \\ 
2023aeas & 10:00:25.818 & +02:18:30.19 & 1.43 (0.07) & 25.90 (0.04) & F115W & 25.90 (0.03) & 1.56 & -- \\ 
2023adzp & 10:00:43.731 & +02:20:18.18 & 1.40 (0.13) & 26.80 (0.06) & F115W & 27.10 (0.07) & -- & -- \\ 
2023aebh & 10:00:37.121 & +02:13:28.53 & 1.39 (0.07) & 25.70 (0.04) & F277W & 27.70 (0.15) & -- & -- \\ 
2023adzn & 10:00:45.601 & +02:20:46.62 & 1.38 (0.14) & 28.00 (0.20) & F150W & 28.00 (0.20) & -- & -- \\ 
2023adzx & 10:00:32.664 & +02:21:19.14 & 1.37 (0.10) & 27.00 (0.08) & F115W & 27.10 (0.07) & 1.19 & 3.39 \\ 
2023aean & 10:00:32.292 & +02:15:15.07 & 1.29 (0.10) & 25.70 (0.05) & F115W & 26.00 (0.04) & -- & 1.27 \\ 
2023aebe & 10:00:34.317 & +02:13:08.65 & 1.11 (0.12) & 26.70 (0.12) & F115W & 27.10 (0.13) & -- & -- \\ 
2023aeai & 10:00:44.004 & +02:14:43.65 & 1.10 (0.11) & 25.20 (0.03) & F115W & 25.40 (0.03) & -- & -- \\ 
2023aebj & 10:00:25.184 & +02:10:52.39 & 1.10 (0.14) & 28.50 (0.22) & F277W & 28.70 (0.34) & -- & -- \\ 
2023adzs & 10:00:24.796 & +02:20:45.70 & 1.09 (0.13) & 26.60 (0.08) & F115W & 26.80 (0.07) & 3.53 & 4.91 \\ 
2023aeac & 10:00:33.613 & +02:24:21.12 & 1.01 (0.13) & 26.40 (0.11) & F115W & 26.90 (0.11) & -- & -- \\ 
2023aebc & 10:00:18.539 & +02:14:52.54 & 1.01 (0.10) & 25.80 (0.04) & F115W & 26.30 (0.04) & -- & -- \\ 
2023aebd & 10:00:30.622 & +02:12:47.26 & 1.01 (0.12) & 26.60 (0.10) & F115W & 26.90 (0.09) & -- & -- \\ 
2023aeba & 10:00:17.348 & +02:17:59.73 & 0.93 (0.15) & 27.30 (0.07) & F277W & 27.40 (0.09) & -- & -- \\ 
2023aeap & 10:00:29.165 & +02:16:01.36 & 0.85 (0.12) & 24.00 (0.02) & F115W & 24.30 (0.02) & -- & -- \\ 
2023adzc & 10:00:24.453 & +02:25:34.08 & 0.70 (0.07) & 25.40 (0.06) & F115W & 25.90 (0.06) & -- & -- \\ 
2023adzj & 10:00:42.116 & +02:22:17.16 & 0.68 (0.10) & 27.20 (0.17) & F115W & 28.00 (0.23) & -- & -- \\ 
2023aeat & 10:00:32.912 & +02:19:02.59 & 0.67 (0.15) & 26.70 (0.08) & F150W & 26.80 (0.09) & -- & -- \\ 
2023adyz & 10:00:41.132 & +02:28:23.49 & 0.65 (0.15) & 25.70 (0.04) & F115W & 26.00 (0.05) & -- & -- \\ 
2023adzm & 10:00:44.261 & +02:24:48.99 & 0.60 (0.14) & 25.10 (0.03) & F115W & 25.20 (0.03) & -- & -- \\ 
2023aeaw & 10:00:28.512 & +02:19:27.67 & 0.59 (0.14) & 27.50 (0.26) & F150W & 27.80 (0.33) & -- & -- \\ 
2023aebm & 10:00:17.478 & +02:14:12.79 & 0.59 (0.15) & 27.90 (0.20) & F150W & 27.90 (0.20) & -- & -- \\ 
2023aeao & 10:00:25.046 & +02:15:41.35 & 0.55 (0.15) & 27.40 (0.17) & F115W & 27.80 (0.16) & -- & -- \\ 
2023aeay & 10:00:17.726 & +02:15:44.07 & 0.55 (0.15) & 26.40 (0.07) & F115W & 26.60 (0.05) & -- & -- \\ 
2023adzz & 10:00:27.114 & +02:22:41.22 & 0.54 (0.15) & 26.70 (0.11) & F115W & 27.40 (0.16) & -- & -- \\ 
2023aeah & 10:00:47.380 & +02:18:03.00 & 0.53 (0.15) & 26.00 (0.06) & F115W & 26.20 (0.05) & -- & -- \\ 
2023adzd & 10:00:28.931 & +02:27:46.92 & 0.49 (0.15) & 25.90 (0.06) & F115W & 26.30 (0.05) & -- & -- \\ 
2023aeau & 10:00:36.637 & +02:19:18.31 & 0.48 (0.14) & 26.00 (0.05) & F115W & 26.10 (0.03) & -- & -- \\ 
2023aebg & 10:00:26.253 & +02:13:26.14 & 0.41 (0.14) & 24.30 (0.02) & F115W & 24.80 (0.02) & -- & -- \\ 
2023adzr & 10:00:27.624 & +02:20:38.05 & 0.39 (0.09) & 25.50 (0.01) & F150W & 25.50 (0.02) & -- & -- \\ 
2023adzh & 10:00:26.997 & +02:25:55.38 & 0.30 (0.13) & 26.90 (0.04) & F150W & 26.90 (0.04) & -- & -- \\ 
2023adzg & 10:00:28.671 & +02:27:23.58 & 0.30 (0.09) & 27.30 (0.13) & F115W & -- & -- & -- \\ 
2023adza & 10:00:28.517 & +02:27:26.43 & 0.30 (0.15) & 26.00 (0.08) & F115W & 26.40 (0.08) & -- & -- \\ 
2023adzb & 10:00:28.763 & +02:27:28.14 & 0.26 (0.13) & 25.60 (0.05) & F115W & 26.00 (0.05) & -- & -- \\ 
2023aeaz & 10:00:17.636 & +02:17:33.73 & 0.25 (0.14) & 27.60 (0.10) & F150W & 27.60 (0.10) & -- & -- \\ 
2023adzf & 10:00:28.030 & +02:28:20.46 & 0.17 (0.07) & 27.30 (0.07) & F150W & 27.30 (0.07) & -- & -- \\ 
2023aear & 10:00:29.417 & +02:17:10.03 & 0.11 (0.05) & 26.00 (0.03) & F115W & 26.10 (0.02) & 1.60 & -- \\ 
2023adzu & 10:00:33.048 & +02:21:00.96 & 0.06 (0.04) & 27.40 (0.07) & F150W & 27.40 (0.07) & -- & -- \\ 
2023aeae & 10:00:36.699 & +02:20:58.98 & 0.06 (0.06) & 26.40 (0.06) & F115W & 27.00 (0.06) & -- & -- \\ 
2023aead & 10:00:37.010 & +02:20:37.63 & 0.06 (0.04) & 27.40 (0.08) & F150W & 28.00 (0.13) & -- & -- \\ 
2023adzk & 10:00:41.600 & +02:24:15.36 & 0.03 (0.06) & 27.90 (0.24) & F150W & 27.90 (0.24) & -- & -- \\ 
2023adzl & 10:00:41.177 & +02:19:47.82 & 0.01 (0.06) & 24.40 (0.01) & F150W & 24.40 (0.01) & -- & -- \\ 
2023adzv & 10:00:28.871 & +02:21:03.58 & 0.01 (0.06) & 28.10 (0.25) & F150W & 28.10 (0.25) & -- & -- \\ 
2023aeaj & 10:00:42.706 & +02:14:59.40 & 0.01 (0.06) & 27.60 (0.14) & F150W & 27.60 (0.14) & -- & -- \\\enddata
\tablecomments{
Column (1): Object name (AT designation). 
Column (2): Right ascension (J2000). 
Column (3): Declination (J2000). 
Column (4): Host photo-redshift with uncertainty (Section \ref{sec:photo-z}). 
%Column (5): Supernova classification (Section \ref{sec:classification}). 
Column (5): Brightest magnitude (AB) with error. 
Column (6): Filter associated with brightest magnitude. 
Column (7): F150W magnitude with error. 
Column (8): Reduced $\chi^2$~value for Type Ia light-curve fit. {\bf Values are not provided when the degrees of freedom are $\leq0$ or for a reduced $\chi^2 > 5$.}
Column (9): Reduced $\chi^2$~value for core–collapse light-curve fit. {\bf Values are not provided when the degrees of freedom are $\leq0$ or for a reduced $\chi^2 > 5$.}
}
\end{deluxetable*}
